Causal-based Time Series Domain Generalization for Vehicle Intention Prediction

Accurately predicting possible behaviors of traffic participants is an essential capability for autonomous vehicles. Since autonomous vehicles need to navigate in dynamically changing environments, they are expected to make accurate predictions regardless of where they are and what driving circumstances they encountered. Therefore, generalization capability to unseen domains is crucial for prediction models when autonomous vehicles are deployed in the real world. In this paper, we aim to address the domain generalization problem for vehicle intention prediction tasks and a causal-based time series domain generalization (CTSDG) model is proposed. We construct a structural causal model for vehicle intention prediction tasks to learn an invariant representation of input driving data for domain generalization. We further integrate a recurrent latent variable model into our structural causal model to better capture temporal latent dependencies from time-series input data. The effectiveness of our approach is evaluated via real-world driving data. We demonstrate that our proposed method has consistent improvement on prediction accuracy compared to other state-of-the-art domain generalization and behavior prediction methods.

==> sections/experiments.tex <==

\section{Experiments}

In this section, we evaluate and compare our method on real-world driving dataset. Results with an in-depth analysis and ablation study are presented in the following.


\subsection{Datasets and Settings}
% talk about how we split domain; difference and similarities between two datasets(how we gonna use them separately); input and output selection. 

The experiment is conducted on the INTERACTION dataset \cite{dataset}, where two different scenarios are utilized: USA\_Roundabout\_FT (an eight-way roundabout in the US) and CHN\_Merging\_ZS (a highway merging scenario in China). All data are collected by a drone from bird’s-eye view with 10 Hz sampling frequency. Information such as reference paths and traffic regulations can be directly extracted from high definition maps that are in lanelet \cite{poggenhans2018lanelet2} format. We further convert each vehicle's state information from Cartesian coordinate to the Fren\'{e}t Frame, in order to deal with domain shift relate to vehicle’s absolute location in the map. 
\begin{figure}[htbp]
	\centering
	\includegraphics[scale=0.4]{map.pdf}
	\caption{Illustration of selected domains for driving scenarios. Three domains selected from USA\_Roundabout\_FT are denoted as FT-1, FT-2, and FT-3. The one domain selected from CHN\_Merging\_ZS is denoted as ZS. Each black arrow line represents a reference path and red circles represent intersect points of reference paths.}
	\label{fig:map}
\end{figure}
\begin{table}[h!]
  \begin{center}
    \caption{Domain generalization results on USA$\_$Roundabout$\_$FT dataset with prediction accuracy (\%).}
    \label{tab:FT_results}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|ccccccc|ccc|c}
      \toprule % <-- Toprule here
      \multicolumn{1}{c|}{} &
	  \multicolumn{7}{c|}{\textbf{Traditional Baseline Methods}} &
	  \multicolumn{3}{c|}{\YH{\textbf{Behavior Prediction Methods}}} &
	  \multicolumn{1}{c}{\textbf{Ours}} \\
      \midrule
      \midrule
      Source & ERM & IRM & CCSA & Mixup & DANN & C-DANN & VRADA & \YH{DESIRE} & \YH{SGAN} & \YH{NRI} & CTSDG \\
      / Target &  \cite{erm} & \cite{irm} & \cite{ccsa} & \cite{mixup} & \cite{dann} & \cite{cdann} & \cite{vrada} & \YH{\cite{DESIRE}} & \YH{\cite{social_GAN}} & \YH{\cite{NRI}} & \\
      \midrule % <-- Midrule here
      1,2 / 3 & 75.97 (2.01) & 82.68 (3.91) & 78.03 (2.26) & 60.70 (16.61) & 77.47 (4.69) & 81.00 (4.87) & 76.35 (10.34) & \YH{75.23 (3.27)} & \YH{74.46 (2.36)} &  \YH{76.34 (1.67)} & 86.03 (1.48) \\
      1,3 / 2 & 97.28 (0.82) & 93.28 (3.83) & 96.68 (1.42) & 94.05 (3.15) & 95.66 (0.77)  & 95.06 (3.48) & 96.43 (0.51) & \YH{95.32 (0.38)} & \YH{94.98 (0.96)} &  \YH{97.01 (0.53)} & 96.85 (0.15) \\
      2,3 / 1 & 98.38 (0.72) & 98.76 (0.20) & 98.29 (0.62) & 91.56 (7.81) & 99.23 (0.34)  & 99.19 (0.45) & 98.12 (0.97) & \YH{96.85 (0.63)} & \YH{99.10 (0.13)} & \YH{98.77 (0.80)}  & 98.85 (0.13) \\
      \midrule
      \multicolumn{1}{c|}{Average} & 90.54 & 91.58 & 91.00 & 82.10 & 90.79 & 91.75 & 90.30 & \YH{89.13} & \YH{89.51} & \YH{90.71} & \textbf{93.91}\\
      %1,2 & 3 & & & & & & & & & \\
      \bottomrule % <-- Bottomrule here
    \end{tabular}}
  \end{center}
\end{table}
In this work, a domain is defined as a driving region that contains a unique combination of road topology, traffic rules, and speed limit information. Three domains are extracted from the FT scenario and one domain is extracted from the ZS scenario (see Figure \ref{fig:map}). %\textcolor{blue}{Talk about how traffic rules are different}




\subsection{Quantitative Results} 
We compare our method with the following \YH{ten state-of-the-art methods, including seven traditional baseline methods for domain generalization tasks and three additional methods for behavior prediction tasks.} (1) \textbf{ERM} \cite{erm} model is trained with cross-entropy loss, without any auxiliary loss. (2) \textbf{IRM} \cite{irm} imposes a regularization term on standard ERM model, to enforce the optimal classifer on top of the representation space to be the same across all domains. (3) \textbf{CCSA} \cite{ccsa} uses semantic alignment to regularize the learned feature subspace for domain generalization. (4) \textbf{Mixup} \cite{mixup} is a data augmentation method that creates out-of-domain samples by applying convex combination to both the input and label space. (5) \textbf{DANN} \cite{dann} adversarially trains the generator and discriminator to learn domain-invariant feature representations.  (6) \textbf{C-DANN} \cite{cdann} is a variation of DANN, where class label is added to the input space for better generalization. (7) \textbf{VRADA} \cite{vrada} combines VRNN and adversarial learning for domain adaptation on time series data. \YH{(8) \textbf{DESIRE} \cite{DESIRE} generates plausible predictions via a conditional variational autoencoder (CVAE)-based RNN encoder-decoder. (9) \textbf{SGAN} \cite{social_GAN} is based on Generative Adversarial Networks (GANs), where the training procedure is a minimax game between a generative model and a discriminative model . (10) \textbf{NRI} \cite{NRI} integrates graph neural network (GNN) into the variational autoencoder (VAE) structure. }

To evaluate the domain generalization performance, we follow the typically used \textit{leave-one-domain-out} protocol \cite{li2017deeper}: multiple domains will be used for model training and the model will be evaluated on the remaining unseen domain. Since most of the baseline models are not designed for time-series input data, for a fair comparison, we add a RNN layer in front of each model instead of simply flattening the time-series input. Moreover, the total numbers of parameters of all the baselines and our method are set to about equal. 

\textbf{Evaluation on USA\_Roundabout\_FT.}
We train all models on different combinations of source domains extracted in FT and report the test results on each corresponding target domain in Table \ref{tab:FT_results}. We observe that our method achieves an average prediction accuracy of 93.91\% under all three train-test domain pairs and increases the accuracy by 2.54\% compared to the best-performed baseline model. \YH{Although DANN, C-DANN, and SGAN slightly outperform CTSDG when FT-1 is chosen as the target domain, their performances are not stable as when other domains are used for testing.} \YH{ERM and NRI method slightly outperform CTSDG when FT-2 is the target domain, but their accuracy is 10.24\% and 11.26\% less than our method when tested on FT-3, respectively.} Moreover, based the worst performance of Mixup, we can conclude that data augmentation methods are not be suitable to vehicle trajectory data, since feasibility constraints cannot be guaranteed in generated data and thus causes performance degradation. As seen, our method has consistent prediction accuracy regardless of testing domains. The standard deviations of CTSDG are also lower than those of all other baseline methods, which further shows our model's efficacy as it converges to more stable local optima. 

%We also notice that the performance of Mixup is the worst compared to other DG methods. The reason is because data augmentation method may generate infeasible vehicle interaction trajectories, which can cause degradation in prediction accuracy. Therefore, applying data augmentation in data that requires to fullfill 




\textbf{Evaluation on CHN\_Merging\_ZS.}
Among the three domains in FT, the domain shift mainly corresponds to changes in road topology and traffic rules. When we compare the domain in ZS with domains in FT, we notice larger difference in road topology as well as in speed limit. In other word, the joint distribution shift is more severe between domains from two different scenarios (i.e. ZS and FT) than domains within scenario FT, which makes domain generalization more challenging. Therefore, in order to evaluate the generalizability of each model under large domain shift, we select different domain combinations in FT for training and the single domain in ZS for testing. 
\begin{table}[h!]
  \begin{center}
    \caption{Domain generalization results on CHN$\_$Merging$\_$ZS dataset with prediction accuracy (\%).}
    \label{tab:ZS_results}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|ccccccc|ccc|c}
      \toprule % <-- Toprule here
      \multicolumn{1}{c|}{} &
	  \multicolumn{7}{c|}{\textbf{Traditional Baseline Methods}} &
	  \multicolumn{3}{c|}{\YH{\textbf{Behavior Prediction Methods}}} &
	  \multicolumn{1}{c}{\textbf{Ours}} \\
      \midrule
      \midrule
      
      Source & ERM & IRM & CCSA & Mixup & DANN & C-DANN & VRADA & \YH{DESIRE} & \YH{SGAN} & \YH{NRI} & CTSDG \\
       & \cite{erm} & \cite{irm} & \cite{ccsa} & \cite{mixup} & \cite{dann} & \cite{cdann} & \cite{vrada} & \YH{\cite{DESIRE}} & \YH{\cite{social_GAN}} & \YH{\cite{NRI}} &\\
      \midrule % <-- Midrule here
      1,2 & 72.71 (3.02) & 75.60 (3.99) & 74.64 (2.61) & 69.08 (6.25) & 77.05 (4.83)  & 76.40 (5.55) & 83.81 (3.57) & \YH{65.32 (2.34)} & \YH{78.02 (5.34)} &  \YH{76.31 (4.49)} & 84.06 (3.54) \\
      1,3 & 80.67 (2.74) & 80.43 (1.92) & 80.92 (5.63) & 79.23 (1.50) & 82.37 (2.54)  & 84.06 (4.35) & 77.54 (6.91) & \YH{70.77 (4.24)} & \YH{78.26 (4.75)} &  \YH{77.23 (4.67)} & 84.78 (3.49) \\
      2,3 & 57.97 (0.73) & 62.80 (1.67) & 61.35 (2.74) & 60.62 (11.55) & 71.50 (13.87)  & 69.56 (10.67) & 68.11 (9.25) & \YH{74.66 (6.03)} & \YH{75.43 (1.51)} &  \YH{75.01 (2.91)} & 77.54 (3.53)\\
      1,2,3 & 80.43 (3.32) & 76.33 (3.72) & 78.02 (3.64) & 70.53 (15.92) & 82.61 (3.16)  & 82.37  (2.54) & 85.02 (2.93) & \YH{73.43 (4.93)} & \YH{83.57 (2.93)} &  \YH{84.10 (3.22)} & 85.51 (2.66) \\
      \midrule
      Average & 72.95 & 73.79 & 73.73 & 69.87 & 78.38 & 78.10 & 78.62 & \YH{71.04} & \YH{78.82} & \YH{78.16} & \textbf{82.97}\\
      %1,2 & 3 & & & & & & & & & \\
      \bottomrule % <-- Bottomrule here
    \end{tabular}}
  \end{center}
\end{table}

We report the result in Table \ref{tab:ZS_results}. We observe that CTSDG consistently outperforms all baseline models across all source-target pairs with accuracy 1\% $\sim$ 6\% higher. \YH{The average prediction accuracy of our method increases by 5\%  compared to the best-performed baseline model. Also, when the model is trained using all three domains in FT, where the source domains have more diversity, learning based methods that do not specifically consider domain generalization approaches (i.e. ERM, DESIRE, SGAN, and NRI) have reasonable performance. However, the performance of ERM and three behavior prediction methods degrade drastically when training data are limited and lack of diversity. Specifically, ERM's and DESIRE's accuracy decreases over 22\% when domain FT-1 and FT-3 is removed from training, respectively.} According to the results, we show the diminishing performance of traditional machine learning model to out-of-training distribution regimes and our proposed method is able to mitigate such problem while consistently outperforms other state-of-the-art methods. 


%each component plays its own role in a complementary way.

\subsection{Further Analysis and Insights}
\textbf{Analysis on Invariant Representation.}
% validate invariant representation: visualization on t-SNE
We utilize t-SNE \cite{t-SNE} to analyze the quality of latent representation learned by our proposed model in Figure \ref{fig:tsne_results}. We train our model using two domains (FT-1,2) and evaluate on two unseen domains (FT-3 \& ZS). It appears from Fig. \ref{fig:tsne_results}(a) and (b) that CTSDG achieved a higher overlap between train and test domains for FT-3 than ZS, highlighting the difficulty of generalizing to the ZS domain. Such finding coincides with our prior domain knowledge as well as quantitative results in Table \ref{tab:FT_results} and Table \ref{tab:ZS_results}. Moreover, based on Fig. \ref{fig:tsne_results}(c) and (d), we find that the classes are well-separated in the training domains for both models. We also observe that when the intention label is \textit{yield}, the data is more evenly dispersed. The reason could because the input time-series data with \textit{yield} label are easier for the model to capture underlying domain representations that are invariant across time. Whereas the time-series data with \textit{pass} label could have more temporally diversed domain-invariant representations. %Both results shows that our model is able to capture temporal latent dependencies 
% Further explain pass and yield label. 
\begin{figure}[htbp]
	\centering
	\includegraphics[scale=0.35]{t-sne.pdf}
	\caption{The t-SNE plots for visualizing latent representations. The source domains come from FT-1 and FT-2. The target domain for (a)-(c) and (b)-(d) is from FT-3 and ZS, respectively. For better visualization, we color (a) and (b) based on domain information: blue dots for FT-1, green dots for FT-2, and red dots for corresponding target domain. In (c) and (d), we color data points by ground-truth vehicle intention labels, where yellow dots represent \textit{pass} and magenta dots represent \textit{yield}.}
	\label{fig:tsne_results}
\end{figure}
\begin{figure}[htbp]
	\centering
	\includegraphics[scale=0.27]{VRNN_results.pdf}
	\caption{Learned temporal latent dependencies across time for different output intentions. The source domains are FT-1,2 and the target domain is FT-3. Each column shows a single sample from either source or target domain. The top row represents the cell state of memory cell for CTSDG, where y-axis refers to the activation of each neuron and x-axis refers to activation per time-step. The second row plots two vehicles' longitudinal coordinates under the Fren\'{e}t Frame with respect to time. The third row plots the velocity profiles for the two interacting vehicles.}
	\label{fig:vrnn_results}
\end{figure}

\textbf{Analysis on Learned Temporal Latent Dependencies.}
% validate temporal latent dependencies: visualization on temporal info
Figure \ref{fig:vrnn_results} shows the temporal latent dependencies learned by our CTSDG for a given source-target pair. We first look at the two cases from source domain (i.e. first column in Fig. \ref{fig:vrnn_results}(a,b)). Looking at the neuron activation patterns along the time axis, we can see that neurons are more active when there are changes in either position or velocity profiles for two interacting vehicles. In fact, these changes are related to causal features which play important roles in determining the output intentions based on our proposed causal model. As we look at the two cases from target domain (i.e. second column in Fig. \ref{fig:vrnn_results}(a,b)), we observe consistent excitatory neuron firing patterns at critical time steps, which indicate that CTSDG successfully transfers knowledge to unseen domains. Therefore, we can conclude that our CTSDG method is able to capture temporal latent dependencies that are domain invariant and related to causal features, which enables it generalize time-series driving data to unseen domains. 













==> sections/extension.tex <==
\YH{\section{Extension to Trajectory Prediction Tasks}}
\YH{In this paper, although we illustrate the performance of our proposed domain generalization method for vehicle intention prediction tasks, our CTSDG approach can also be directly or indirectly utilized for trajectory prediction tasks. The most straight forward way is to frame the trajectory prediction problem as classification over a diverse set of trajectories.  In fact, according to \cite{phan2020covernet}, by framing trajectory prediction problem as classification over a diverse set of trajectories, we were able to a) ensure a desired level of coverage of the state space, b) eliminate dynamically infeasible trajectories, and c) avoid the issue of mode collapse. }

\YH{Moreover, the accuracy of intention classification plays an important role in regression tasks. As stated and showed in \cite{TNT, deo2018multi, goal_plan_predestrain, ITSC_ttlc},  goal/intent-conditioned trajectory forecasting can improve joint-agent and per-agent predictions, compared to unconditional forecast. Conditional forecasting can be also used for planning tasks, which effectiveness is demonstrated in \cite{Precog}. Therefore, having an accurate and domain generalizable intention/goal predictor is the prerequisite of developing state-of-the-art trajectory predictor and motion planner.}


==> sections/introduction.tex <==
\section{Introduction}

Researchers have developed various machine learning algorithms to enhance the accuracy of intention and motion prediction tasks for autonomous vehicles \cite{zhang2013understanding, pass_yield_merge_PGM, ITSC_DBN_intent, roundabout_RNN_intent_traj, Intentnet, TNT, DESIRE, Precog, Traffic}. Although these machine learning algorithms provide excellent prediction performance, a key assumption underlying the remarkable success is that the training and test data usually follow similar statistics. Otherwise, when test domains are unseen or Out-of-Distribution (OOD) \cite{OOD_AV}, the resulting train-test domain shift leads to significant degradation in prediction performance. Incorporating data from multiple training domains somehow alleviates this issue \cite{li2017deeper}. However, this may not always be applicable as it can be overwhelming to collect data from all the domains, especially for autonomous driving. 

\YH{The area of domain adaptation (DA) \cite{DA_1,DA_2,DA_3} aims to alleviate the aforementioned problem by assuming unlabeled target domain data is accessible at the training stage and adapting models to the testing domain.} However, data may not be available for the target domain and we expect great prediction performances even when unseen domains are encountered. Therefore, domain generalization (DG) comes into place, where it aims to build or train models that are designed for increased robustness to domain-shift without requiring access to target domain data.
Many researchers have been working on developing DG algorithms \cite{ghifary2015domain, li2018domain, li2018learning, balaji2018metareg, carluccidomain, cdann, causal_1, MatchDG, causal_2, mixup}, but most of these models are designed for tasks such as object recognition, semantic segmentation, image classification, and disease detection. In this paper, our goal is to design a DG algorithm for vehicle intention prediction task which is different from typical DG tasks in three aspects: (1) the input is numerical time-series data instead of static image; (2) each input data point contains information of multiple agents (e.g. vehicles) with interactions involved, instead of a single agent (e.g. patient) with no interaction; (3) factors that cause domain shift are ambiguous for our task, in contrast to clear domain shift variables for other DG tasks (e.g. image rotation angle or style for image classification task). Therefore, directly applying state-of-the-art DG approaches may not be suitable for our problem setting and could result in undesirable performance. It is thus necessary to develop a domain generalization model that considers the discrepancies in the aforementioned aspects and is applicable for vehicle intention prediction task.

According to \cite{causal_review}, causality, with its focus on representing structural knowledge about the data generating process that allows interventions and changes, can contribute towards understanding and resolving some limitations of current machine learning methods. In fact, machine learning models that incorporate or learn structural knowledge of an environment have been shown to be more efficient and generalize better \cite{battaglia2016interaction, bapst2019structured, battaglia2018relational, santoro2017simple}. For human drivers, the way they interact with each other under different domains should also processes some invariant structural relations, since they can quickly adapt their driving skills to novel scenarios. Therefore, we construct a structural causal model (SCM) for vehicle intention prediction task to learn an invariant representation of input driving data for domain generalization. We further integrate a recurrent latent variable model into our structural causal model to better capture temporal latent dependencies from time-series input data. 

In this paper, a causal-based time series domain generalization (CTSDG) model for vehicle intention prediction is proposed. To the best of our knowledge, this is the first work trying to tackle time series domain generalization problem for vehicle intention prediction task. The effectiveness of our approach is evaluated on real-world driving data under different scenarios. Our method also shows consistent improvement on prediction accuracy compared to other state-of-the-art domain generalization methods. 




% First talk about the advantages of causal learning and how it suits well in our settings (e.g. we have some prior knowledge). Then talk how to use VRNN to capture temporal latent dependncies (due to its advantages such as ....) and integrate it into our causal model. 


% \begin{itemize}
%     \item Moreover, we assume that each input data is constructed from a mix of inherent (causal) and domain-dependent (non-causal) features. Consequently, the captured temporal latent dependencies from sequential data also contain both causal and non-causal features. Therefore, we construct a structural causal model inspired from data generation process and propose to learn an invariant representation from temporal latent dependencies of input data for domain generalization, where the learning scheme is based on an invariant condition identified from the causal model.
    
%     \item In this paper, we propose to learn a common representation of time-series data that can be transferred across domains. Specifically, we first use variational methods to produce a latent representation that captures underlying temporal latent dependencies in the data. We then utilize a structural causal model to identify a correct invariant condition needed for our domain generalization task and extract corresponding causal (domain-independent) features from the previously learned latent representation.
    
%     \item To the best of our knowledge, this is the first model trying to tackle time series domain generalization problem for vehicle intention prediction task. 
%     \item Specifically, based on a structural causal model, we proposed to learn an invariant representation for time series vehicle interaction data and utilize the learned representation for domain generalization. 
    
%     \item The causal approach makes these assumptions more explicit and aligned with our understanding of physics and human cognition, for instance
    
%     \item Machine learning models that incorporate or learn structural knowledge of an environment have been shown to be more efficient and generalize better \cite{xx}. In a modular representation of the world where the modules correspond to physical causal mechanisms, many modules can be expected to behave similarly across different tasks and environments. An agent facing a new environment or task may thus only need to adapt a few modules in its internal representation of the world \cite{xx}. When learning a causal model, one should thus require fewer examples to adapt as most knowledge, i.e.,modules, can be re-used without further training.
    
%     \item In \cite{xx}, the authors argue that causality, with its focus on representing structural knowledge about the data generating process that allows interventions and changes, can contribute towards understanding and resolving some limitations of current machine learning methods.
% \end{itemize}


==> sections/method.tex <==
\section{Method}
% we utilize cause representation learning
In this section, we present the details of our proposed Causal-based Time Series Domain Generalization (CTSDG) model, which captures and transfers inter-vehicle causal relations as well as temporal latent dependencies across domains via domain-invariant representations.

\subsection{Notations}
%talk about how we define domain
Let $\mathcal{X}$ be the input space and $\mathcal{Y}$ the label space, a \textit{domain} is defined as a joint distribution $P_{XY}$ on $\mathcal{X} \times \mathcal{Y}$. In the context of domain generalization, we assume to have access to $K$ domains, $\mathcal{D} = \{D_k\}^{K}_{k=1}$, each associated with a joint distribution $P_{XY}^{k}$. In each domain, data-label pairs are sampled from a dataset $D_k = \{(\mathbf{x}_i^{(k)},\mathbf{y}_i^{(k)})\}_{i=1}^{N_k}$ with $(\mathbf{x}_i^{(k)},\mathbf{y}_i^{(k)}) \sim P_{XY}^{k}$, where $N_k$ is the number of labeled data points in the $k$-th domain and $\mathbf{x}_i = (x_t^i)_{t=1}^{T} = ([\xi_t^{A,i}, \xi_t^{B,i}])_{t=1}^T$ denotes a multivariate time series with $x_t^i \in \mathbb{R}^{H \times 2}$. For a given
vehicle, we use $\xi$ to represent historical trajectories. \YH{In this work, given historical trajectories of interacting vehicle pairs (i.e. car A and car B), the domain generalization task is to learn an intention predictor $f$ (i.e. predict interaction outcomes such as pass/yield) that generalizes well to unseen target domains $k' \notin D_k$ where $P_{XY}^{(k')} \neq P_{XY}^{(k)}$, $\forall k \in \{1,\dots,K\}$.} %However, unlike domain adaptation, domain generalization assumes no explicit knowledge about the target distribution. %which may have large discrepancy from the training distribution. 
%Therefore, if the standard empirical risk minimization (ERM) is used, it can overfit to the training domains. 


\subsection{Learning Invariant Representation from Causal Model}
%The domain generalization setting assumes the existence of domain-invariant patterns in the inputs (e.g. semantic features), which can be extracted to learn a predictor that performs well across seen and unseen domains. \textcolor{blue}{Also, as discussed in Section XX (related work) (talk about the advantages of causal model)}.

In this work, we propose a causal view of data generating process under vehicle interaction settings. More specifically, we utilize a structural causal model (SCM) based on domain knowledge to describe how interactive trajectories are generated by any vehicle pair (see Figure \ref{fig:framework}). The constructed causal structure provides us with causal relations between input features and the outcome, which is used to learn the intention predictor. The detailed meaning of each node variable is listed below:\\
\-\hspace{0.5cm}\textbf{Domain ($D$)} contains different combinations of map properties such as road topology, speed limit, and traffic rules.\\
\-\hspace{0.5cm}\textbf{Event ($E$)} denotes an observable variable relate to the event of two-vehicle interaction, which includes information such as initial interaction states and the length of interaction.\\
\-\hspace{0.5cm}\textbf{Driver ($O$)} denotes an unobservable variable relate to each driver's driving preferences or style, such as the aggressiveness level and whether he/she obeys traffic rules.\\
\-\hspace{0.5cm}\textbf{Causal features} ($X_C$) represent high-level time-related causal features derived from drivers' personal behavior $O$ and their interaction status $E$, which are used by humans to label the intention.\\
\-\hspace{0.5cm}\textbf{Non-causal features} ($X_{NC}$) represent domain dependent features which contain not only domain-specific information $D$, but also event $E$. For example, interaction event information such as when two vehicles start noticing each other or when the road negotiation begins, is related to the road geometry and traffic rule. \\
\-\hspace{0.5cm}\textbf{Input Data} ($X$) is vehicle interactive trajectories that contain sequential multivariate data, and is constructed from a mixture of causal $X_C$ and non-causal $X_{NC}$ features.\\
\-\hspace{0.5cm}\textbf{Latent variable} ($Z$) denotes time-related latent representations extracted from time-series vehicle interaction data.\\
\-\hspace{0.5cm}\textbf{Label} ($Y$) is the vehicle intention label. For two vehicle interaction cases, we normally assign a binary label to represent selected vehicle's intention of either passing or yielding the other vehicle at a given time step.


%Each pair of interactive trajectories is obtained by first selecting two vehicles in a scene (i.e. domain $D$) that have potential interaction with each other and the unobservable drivers' information are stored in $O$. Then, a desired starting time and interaction period (i.e. variables related to $E$) are selected. The driving scenario corresponds to domain-depended high-level features $X_{NC}$. Both $O$ and $E$ correspond to high-level causal features $X_C$ which are used by human to label the intention $Y$. Finally, $X_C$ and $X_{NC}$ construct the interactive trajectories $X$. 

\textbf{Invariance Condition.} According to Figure~\ref{fig:framework}, $X_C$ is the node that causes $Y$, and by d-separation \cite{pearl2009causality}, the intention label is independent of domain conditioned on $X_C$, $Y \ind D | X_C$\footnote{The notation $Y \ind D | X_C$ stands for the conditional independence relationship $P(Y = y, D = k| X_C = \mathbf{x}_c) = P(Y = y| X_C = \mathbf{x}_c)P(D = k|X_C = \mathbf{x}_c)$.}. In other word, if such a $X_C$ can be found, then the
distribution of Y conditional on $X_C$ is invariant under transferring from the source domains to the target domains. Therefore, our intention prediction task is to learn $y$ as $h(\mathbf{x}_c)$ where $h: \mathcal{C} \rightarrow \mathcal{Y}$. However, since $X_C$ is unobserved, we need to learn $y$ through observed trajectories $X$. Specifically, we utilize a representation function $q: \mathcal{X} \rightarrow \mathcal{Z}$ to map the input space to a latent space, and a hypothesis function $\phi: \mathcal{Z} \rightarrow \mathcal{C}$ to map the latent space to $X_C$. Together, $h(\phi(q(\mathbf{x})))$ leads to the desired intention predictor $f: \mathcal{X} \rightarrow \mathcal{Y}$ and the corresponding prediction loss can be written as:
\begin{equation}\label{eq:L_y}
    \mathcal{L}_y = \mathcal{L}_\alpha(h(\phi(q(X))), Y),
\end{equation}
where $\mathcal{L}_\alpha$ is the classification loss such as a binary or categorical cross-entropy. In addition, by d-separation, $X_C$ also needs to satisfy an invariance condition: $X_C \ind D|\{E, O\}$, which means $X_C$ does not change with different domains when both event and driver information remain the same. However, driver information is unobservable and in many dataset there may not be an exact match based on a same interaction event across domains. Alternatively, we assume that the distance over $X_C$ between same-class inputs from different domains is bounded, which provides an alternative invariance condition that is consistent with the conditional independencies of $X_C$. %If a dataset has low $\delta$, then there is a high chance of learning a good representation that is close to $X_C$. 
Therefore, we would like to minimize the following objective along with the prediction loss:
\begin{equation}\label{eq:L_r}
    \mathcal{L}_r = \sum_{\Omega(\mathbf{x}_j,\mathbf{x}_m)=1; k_j \neq k_m}\mathcal{L}_\beta(\phi(q(\mathbf{x}_j^{(k_j)})), \phi(q(\mathbf{x}_m^{(k_m)}))),
\end{equation}
where $\mathcal{L}_\beta$ is the distance metric such as $\ell_2$, and $\Omega: \mathcal{X} \times \mathcal{X} \rightarrow \{0, 1\}$ is a match function such that pairs having $\Omega(\mathbf{x}_j, \mathbf{x}_m) = 1$ have low difference in their causal features.

\textbf{Contrastive Representation Learning.} To optimize $\mathcal{L}_r$, we first need to learn a proper match function $\Omega$ used in Eq.~(\ref{eq:L_r}). Specifically, we optimize a contrastive representation learning loss that minimizes distance between same-class inputs from different domains. We regard positive matches as two inputs from the same class but different domains, and negative matches as pairs with different classes. Then the loss function for every positive match pair $(j, m)$ in a sampled mini-batch $\mathcal{B}$ is defined as:
\begin{eqnarray}\label{eq:contrast_loss}
    \ell^{j,m}_{con} = -\log\frac{\mathrm{exp}(s_{cos}(\mathbf{x}_j, \mathbf{x}_m)/\tau)}{\mathrm{exp}(s_{cos}(\mathbf{x}_j, \mathbf{x}_m)/\tau) + \sum_{i=1, y_i \neq y_j}^{|\mathcal{B}|}\mathrm{exp}(s_{cos}(\mathbf{x}_j, \mathbf{x}_i)/\tau)},
\end{eqnarray}
where $s_{cos}(\mathbf{x}_a, \mathbf{x}_b) = \phi(q(\mathbf{x}_a))^T\phi(q(\mathbf{x}_b))/\|\phi(q(\mathbf{x}_a))\| \|\phi(q(\mathbf{x}_b))\|$ is the inner product of two $\ell_2$-normalized vectors, $\tau$ is a temperature scaling parameter, and $|\mathcal{B}|$ is the batch size. Inspired from \cite{MatchDG}, for this unsupervised contrastive learning process, we initialize $\Omega$ with a random match based on classes and keep updating $\Omega$ by minimizing the contrastive loss (\ref{eq:contrast_loss}) until convergence.


\subsection{Capturing Temporal Latent Dependencies}
%As discussed earlier, simply using deep learning models like RNN cannot efficiently model complex dependencies ...\textcolor{blue}{From our SCM, we observe that $Z \ind D | X$. Talk about the relation with previously mentioned representation function q}.
From our proposed causal model in Fig.\ref{fig:framework}, we also observe that $Z \ind D | X$, meaning the latent representation is independent of domain $D$ conditioned on input data $X$. Therefore, by learning the representation function $q$, we are able to extract a domain-invariant latent variable that represents the input space. Since the input is time-series data, the learned latent variable is expect to capture temporal latent information in the data. To explicitly model the dependencies between latent random variable across time steps, we integrate Variational Recurrent Neural Networks (VRNN) into our CTSDG model. It is verified in \cite{VRNN} that VRNN can model highly structured sequential data better than other RNN-based model by the introduction of latent random variables. The VRNN contains a VAE at every time step and these VAEs are conditioned on previous auto-encoders via the hidden  state variable $h_{t-1}$ of an RNN. Therefore, for each time step of $x_t^i$, a latent random variable $z_t^i$ is learned following the equation $z_t^i|x_t^i \sim \mathcal{N}(\mu_{z,t}, \mathrm{diag}(\sigma_{z,t}))$, where $[\mu_{z,t}, \sigma_{z,t}] = \varphi_\tau^{enc}(\varphi_\tau^{x}(x_t^i), h_{t-1})$. The prior $z_t^i$ is derived from $z_t^i \sim \mathcal{N}(\mu_{0,t}, \mathrm{diag}(\sigma_{0,t}))$, where $[\mu_{0,t}, \sigma_{0,t}]= \varphi_\tau^{prior}(h_{t-1})$. Variables $\mu_{*,t}$ and $\sigma_{*,t}$ denote parameters of a generating distribution, and $\varphi_\tau^*$ can be any highly flexible function (e.g. deep neural network) with corresponding parameter set $\tau$. Moreover, $x_t^i$ is not only conditioned on $z_t$ but also on $h_{t-1}$ such that $x_t^i|z_t^i \sim \mathcal{N}(\mu_{x,t}, \mathrm{diag}(\sigma_{0,t}))$, where  $[\mu_{x,t}, \sigma_{x,t}] = \varphi_\tau^{dec}(\varphi_\tau^{z}(z_t^i), h_{t-1})$. In general, the objective function become a timestep-wise variational lower bound:
\begin{equation}\label{eq:L_v}
    \begin{split}
        \mathcal{L}_{v} = \mathbb{E}_{q(z_{\leq T}^i|x_{\leq T}^i)}[\sum_{t=1}^{T}(-\text{KL}(q(z_t^i|x_{\leq t}^i, z_{\leq t}^i)||p(z_t^i|x_{< t}^i, z_{< t}^i)) +\log p(x_t^i|z_{\leq t}^i, x_{\leq t}^i))],
    \end{split}
\end{equation}
where $q(z_t^i|x_{\leq t}^i, z_{\leq t}^i)$ is the inference model, $p(z_t^i|x_{< t}^i, z_{< t}^i))$ is the prior, $p(x_t^i|z_{\leq t}^i, x_{\leq t}^i)$ is the generative model, and $\text{KL}(\cdot||\cdot)$ refers to Kullback-Leibler divergence. 

\subsection{Implementation}
Combining the joint optimization problem of equation (\ref{eq:L_y}), (\ref{eq:L_r}), and (\ref{eq:L_v}) leads to our CTSDG model. The complete objective function we aim to optimize is:
\begin{equation}\label{eq:L}
    \mathcal{L} = \mathcal{L}_y + \gamma \mathcal{L}_v + \lambda \mathcal{L}_r,
\end{equation}
where $\gamma$ and $\lambda$ are hyperparameters that control training balance among three losses for better performance. In order to prevent the classification loss from interfering learning domain-invariant representations, we learn the match function $\Omega$ before optimizing the overall objective function (\ref{eq:L}). Also, since the causal feature $X_C$ is a function of latent variable $Z$ which is extracted by the recurrent latent variable model, the objective function (\ref{eq:L_v}) needs to be jointly optimized while learning the matching function using Eq.(\ref{eq:contrast_loss}). 
% Briefly talk about the networks and training schemes
% Add a table for the overall algorithm

==> sections/motivation.tex <==
\section{Problem Statement}
Figure~\ref{fig:motivation} illustrates the motivation of this work. Consider two vehicles interact with each other under two different scenarios. For better understanding of the concept, we temporarily make the following assumptions\footnote{The last two assumptions will not be made in the rest of this paper since they are hard to hold when data are collected in the real world. The first assumption will still be considered.} for both interaction cases: 
\begin{itemize}
    \item Same relative road priority of two roads that two vehicles are driving on.
    \item Same drivers driving the two cars, whose driving styles are consistence across different scenarios \cite{xx}.
    \item Same distance towards two roads' conflict/intersect point (i.e. black dot) for both vehicles when interaction begins.
\end{itemize}
There are also two main differences between two cases: (1) Different topological road structure of two intersected roads, which can be regarded as different domains; (2) Two drivers have different driving styles and the driver in the red car is more aggressive than the driver in the blue car, which information is actually unavailable when making predictions. 

Based on previous assumptions and settings, for a given interaction period, a plausible velocity profile of two vehicles is shown in the second row of Fig.~\ref{fig:motivation} for both cases. The goal is to predict the intention of any selected vehicle, which can be the intent of passing or yielding the other car. According to the plots, whether the red car yields or passes the blue car doesn't relate much to the domain information but depends more on two drivers' personal information (e.g. driving style) and their initial states. Specifically, the geometry of the roads could affect several factors such as when two vehicles start noticing each other, when the road negotiation begins, and when drivers agree on who will go first. All these factors could then influence the velocity profiles of two vehicles but won't have much effects on the intention of two vehicles when the aforementioned assumptions hold. In other words, if two vehicles encounter each other twice under different domains, as long as the three assumptions are true, the aggressive driver will always prefer passing than yielding the less aggressive driver.

Therefore, it is the features that relate to two drivers' information and their internal relations  (e.g. highlighted in cyan), instead of those that relate to domain itself (e.g. highlighted in orange),  determine the intention. Hence, we construct a model for the data collection process that assumes each input data (i.e. vehicle trajectories) is constructed from a mix of causal and non-causal features. We consider domain as a main intervention that changes the non-causal features of an input data, and propose that an ideal intention predictor should depends only on the causal features.

==> sections/problem_setting.tex <==
\section{Problem Setting and Notions}

==> sections/related_works.tex <==
\section{Related Works}

%\textbf{Domain Adaptation}
% talk about the general concept and how it is not align with our case

\textbf{Domain generalization}
% talk about different types of method in DG and the advantages of causal learning \cite{Bengio}. especially talk about why our problem setting works best using such method
% talk about most work is done in non timeseries data. Recent works in time-series data. 
% -> The domain generalization setting assumes the existence of domain-invariant patterns in the inputs (e.g. semantic features), which can be extracted to learn a predictor that performs well across seen and unseen domains. 
aims to generalize models to unseen domains without knowledge about the target distribution during training. Different methods have been proposed for learning generalizable and transferable representations. A commonly-used strategy is to extract task-specific but domain-invariant features \cite{ghifary2015domain, li2018domain, cdann, causal_1, MatchDG, causal_2}. Ghifary et al. \cite{ghifary2015domain} learn multi-task auto-encoders to extract invariant features which are robust to domain variations. Li et al. \cite{li2018domain}
extend adversarial autoencoders by imposing maximum mean discrepancy measure to align multi-domain distributions. Li et al. \cite{cdann} consider the conditional distribution of label space over input space, and minimize discrepancy of a joint distribution. Recently, several works \cite{causal_1, MatchDG, causal_2} utilize causal structures to learn invariance factors, which have shown better model generalizability on unseen data, especially on data from different distributions than the train distribution. 

Dataset augmentation is another strategy that focuses on creating more out-of-domain samples by adversarially perturbing samples \cite{volpi2018generalizing}, leveraging self-supervised signals \cite{carluccidomain}, or utilizing convex combinations of input and output data \cite{mixup}. These data augmentation methods have shown effective for model generalization, but invalid samples could be generated and degrade the model performance if input data is vehicle trajectories that need to satisfy feasibility constraints. Meta-learning can also be applied in domain generalization, by creating meta-train and meta-test sets, and training a model using the meta-train set in such a way to improve the performance on the meta-test set \cite{finn2017model, li2018learning, balaji2018metareg}. While our proposed method can achieve promising results using standard training schemes, combining meta-learning with our approach could be an interesting future direction. 

\begin{figure*}[htbp]
	\centering
	\includegraphics[scale=0.5]{framework.pdf}
	\caption{Illustration of the overall CTSDG framework. Observed quantities are shown as shaded nodes; nodes of latent quantities are transparent. A directed black edge ($\rightarrowRHD$) denotes a causal relationship; dashed bidirectional edges ($\dashbiarrow$) denote correlation; hollow dashed arrows ($\hollowdasharrow$) denote an inclusion relationship. Blue lines ($\bluearrow$) denote the inference process, $q(z_t|x_{\leq t}, z_{< t})$; green lines ($\greenarrow$) represent the generation process, $p(x_t|z_{\leq t}, x_{<t})$; red lines ($\redarrow$) show the recurrence process where $h_t$ is informed by $h_{t-1}$, which is informed by $z_{t-1}$ and $x_{t-1}$.}
	\label{fig:framework}
\end{figure*}

\textbf{Intention prediction in autonomous driving}
aims to predict high-level behaviors of road entities, which results are often used in downstream trajectory prediction modules. \YH{For example, works such as \cite{deo2018multi}, \cite{goal_plan_predestrain} and \cite{ITSC_ttlc} demonstrate that by predicting  goal  states  and  assuming  that  agents  navigate toward  those  goals  by  following  some  optimal  or  learned trajectories, the accuracy of prediction can be improved.} Therefore, accurate intention prediction algorithm is essential for autonomous vehicles to smoothly navigate in dynamic environments. Zhang et al. \cite{zhang2013understanding} propose to model high level semantics in the form of traffic patterns through a generative model. Dong et al. \cite{pass_yield_merge_PGM} use a probabilistic graphical model to estimate the pass or yield probability under merging scenarios. Schulz et al. \cite{ITSC_DBN_intent} utilize the dynamic bayesian network method for routing prediction at intersections. Zyner et al. \cite{roundabout_RNN_intent_traj} obtain a probability distribution over all possible exit branches for a vehicle driving in a roundabout using recurrent neural network. Works such as \cite{Intentnet} and \cite{TNT}, use more complication ML models to prediction vehicle's intention. Due to the complexity of the real-world and its ever-changing dynamics, the deployed autonomous vehicles inevitably face novel situations and should be able to cope with them. However, it has been repeatedly demonstrated that the reliability of ML models degrades radically when they are exposed to novel settings (i.e., under a shift away from the distribution of observations seen during their training) due to their failure to generalize, leading to catastrophic outcomes \cite{amodei2016concrete, sugiyama2012machine}. In \cite{OOD_AV}, Filos et al. also demonstrate that several state-of-the-art behavior prediction models for autonomous driving fail to generalize under arbitrary domain shift. Therefore, in this paper, we aim to address the domain generalization problem for vehicle intention prediction task and provide an effective solution to enhance reliability of autonomous vehicles. We hope our work can inspire further research in the field of improving generalizability for prediction algorithms in autonomous driving industry. 

%We hope our work could draw attention to more researchers and 
